A Month in the Life of Groupon

Groupon has become the latest Internet sensation, providing daily deals to customers in the form of discount offers for restaurants, ticketed events, appliances, services, and other items. We undertake a study of the economics of daily deals on the web, based on a dataset we compiled by monitoring Groupon over several weeks. We use our dataset to characterize Groupon deal purchases, and to glean insights about Groupon's operational strategy. Our focus is on purchase incentives. For the primary purchase incentive, price, our regression model indicates that demand for coupons is relatively inelastic, allowing room for price-based revenue optimization. More interestingly, mining our dataset, we find evidence that Groupon customers are sensitive to other, "soft", incentives, e.g., deal scheduling and duration, deal featuring, and limited inventory. Our analysis points to the importance of considering incentives other than price in optimizing deal sites and similar systems.

==> conclusion.tex <==
\vspace{-1em}
\section{Conclusion and Future Work}

Our work to date has characterized customer purchases of daily 
deals offered by Groupon, and has investigated relationships 
between price, other key deal attributes, and deal size.  One
key outcome of our modeling work is preliminary evidence that 
Groupon is behaving strategically to optimize deal offerings, 
giving customers ``soft'' incentives to purchase.  

One specific line of our future work regards the predictability of 
deal sizes.  How early in the day can we obtain strong predictions 
of the final deal size based on sales thus far and our time-series 
data, and how does this compare with our zero hour prediction?
%%%before the deal is even underway.  
Another line examines the interplay
between social networks and deal purchases.  To what extent does
sharing of information through social networks increase Groupon
sales, and do existing propagation models, 
%%of dissemination on social networks
such as the Independent Cascade model~\cite{Kempe2003Maximizing}, apply?


==> related.tex <==
%%\section{Related Work}

\smallskip

\noindent{\bf Related Work: } To date, there has been little previous work
examining Groupon specifically. Edelman et al. consider the benefits and
drawbacks of using Groupon from the side of the merchant, modeling whether the
advertising and price discrimination effects can make such discounts
profitable~\cite{Edelman2010To}. Dholakia polls businesses to determine their
experience of providing a deal with Groupon~\cite{Dholakia2010How}, and
Arabshahi examines their business model~\cite{Arabshahi2010Undressing}.
Several works have studied other online group buying schemes that arose before
Groupon, and that utilize substantially different dynamic pricing schemes
\cite{Anand2003Group,Kauffman2001New}.


